Compressed Covariance Estimation With Automated Dimension Learning

We propose a method for estimating a covariance matrix that can be represented as a sum of a low-rank matrix and a diagonal matrix. The proposed method compresses high-dimensional data, computes the sample covariance in the compressed space, and lifts it back to the ambient space via a decompression operation. A salient feature of our approach relative to existing literature on combining sparsity and low-rank structures in covariance matrix estimation is that we do not require the low-rank component to be sparse. A principled framework for estimating the compressed dimension using Stein's Unbiased Risk Estimation theory is demonstrated. Experimental simulation results demonstrate the efficacy and scalability of our proposed approach.

==> referencesup.tex <==
@article{anderson1984multivariate,
  title={Multivariate statistical analysis},
  author={Anderson, TW},
  journal={VVi11ey and Sons, New York, NY},
  year={1984}
}
@article{werner2008estimation,
  title={On estimation of covariance matrices with Kronecker product structure},
  author={Werner, Karl and Jansson, Magnus and Stoica, Petre},
  journal={IEEE Transactions on Signal Processing},
  volume={56},
  number={2},
  pages={478--491},
  year={2008},
  publisher={IEEE}
}
@article{pourahmadi2011covariance,
  title={Covariance estimation: The GLM and regularization perspectives},
  author={Pourahmadi, Mohsen},
  journal={Statistical Science},
  pages={369--387},
  year={2011},
  publisher={JSTOR}
}
@article{kaufman2008covariance,
  title={Covariance tapering for likelihood-based estimation in large spatial data sets},
  author={Kaufman, Cari G and Schervish, Mark J and Nychka, Douglas W},
  journal={Journal of the American Statistical Association},
  volume={103},
  number={484},
  pages={1545--1555},
  year={2008},
  publisher={Taylor \& Francis}
}
@article{smith2002parsimonious,
  title={Parsimonious covariance matrix estimation for longitudinal data},
  author={Smith, Michael and Kohn, Robert},
  journal={Journal of the American Statistical Association},
  volume={97},
  number={460},
  pages={1141--1153},
  year={2002},
  publisher={Taylor \& Francis}
}
@article{bai2011estimating,
  title={Estimating high dimensional covariance matrices and its applications},
  author={Bai, Jushan and Shi, Shuzhong and others},
  journal={Annals of Economics and Finance},
  volume={12},
  number={2},
  pages={199--215},
  year={2011},
  publisher={Society for AEF}
}
@article{witten2009penalized,
  title={A penalized matrix decomposition, with applications to sparse principal components and canonical correlation analysis},
  author={Witten, Daniela M and Tibshirani, Robert and Hastie, Trevor},
  journal={Biostatistics},
  pages={kxp008},
  year={2009},
  publisher={Biometrika Trust}
}
@article{shen2008sparse,
  title={Sparse principal component analysis via regularized low rank matrix approximation},
  author={Shen, Haipeng and Huang, Jianhua Z},
  journal={Journal of multivariate analysis},
  volume={99},
  number={6},
  pages={1015--1034},
  year={2008},
  publisher={Elsevier}
}
@article{goldfarb2003robust,
  title={Robust portfolio selection problems},
  author={Goldfarb, Donald and Iyengar, Garud},
  journal={Mathematics of operations research},
  volume={28},
  number={1},
  pages={1--38},
  year={2003},
  publisher={INFORMS}
}
@article{engle1981one,
  title={A one-factor multivariate time series model of metropolitan wage rates},
  author={Engle, Robert and Watson, Mark},
  journal={Journal of the American Statistical Association},
  volume={76},
  number={376},
  pages={774--781},
  year={1981},
  publisher={Taylor \& Francis Group}
}
@article{chen2013covariance,
  title={Covariance and precision matrix estimation for high-dimensional time series},
  author={Chen, Xiaohui and Xu, Mengyu and Wu, Wei Biao and others},
  journal={The Annals of Statistics},
  volume={41},
  number={6},
  pages={2994--3021},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{basu2015regularized,
  title={Regularized estimation in sparse high-dimensional time series models},
  author={Basu, Sumanta and Michailidis, George and others},
  journal={The Annals of Statistics},
  volume={43},
  number={4},
  pages={1535--1567},
  year={2015},
  publisher={Institute of Mathematical Statistics}
}
@article{xiao2012covariance,
  title={Covariance matrix estimation for stationary time series},
  author={Xiao, Han and Wu, Wei Biao and others},
  journal={The Annals of Statistics},
  volume={40},
  number={1},
  pages={466--493},
  year={2012},
  publisher={Institute of Mathematical Statistics}
}
@article{mcmurry2010banded,
  title={Banded and tapered estimates for autocovariance matrices and the linear process bootstrap},
  author={McMurry, Timothy L and Politis, Dimitris N},
  journal={Journal of Time Series Analysis},
  volume={31},
  number={6},
  pages={471--482},
  year={2010},
  publisher={Wiley Online Library}
}
@article{hamill2001distance,
  title={Distance-dependent filtering of background error covariance estimates in an ensemble Kalman filter},
  author={Hamill, Thomas M and Whitaker, Jeffrey S and Snyder, Chris},
  journal={Monthly Weather Review},
  volume={129},
  number={11},
  pages={2776--2790},
  year={2001}
}
@article{furrer2006covariance,
  title={Covariance tapering for interpolation of large spatial datasets},
  author={Furrer, Reinhard and Genton, Marc G and Nychka, Douglas},
  journal={Journal of Computational and Graphical Statistics},
  volume={15},
  number={3},
  pages={502--523},
  year={2006},
  publisher={Taylor \& Francis}
}
@article{houtekamer2001sequential,
  title={A sequential ensemble Kalman filter for atmospheric data assimilation},
  author={Houtekamer, Peter L and Mitchell, Herschel L},
  journal={Monthly Weather Review},
  volume={129},
  number={1},
  pages={123--137},
  year={2001}
}
@article{zou2006sparse,
  title={Sparse principal component analysis},
  author={Zou, Hui and Hastie, Trevor and Tibshirani, Robert},
  journal={Journal of computational and graphical statistics},
  volume={15},
  number={2},
  pages={265--286},
  year={2006},
  publisher={Taylor \& Francis}
}
@article{d2008first,
  title={First-order methods for sparse covariance selection},
  author={d'Aspremont, Alexandre and Banerjee, Onureena and El Ghaoui, Laurent},
  journal={SIAM Journal on Matrix Analysis and Applications},
  volume={30},
  number={1},
  pages={56--66},
  year={2008},
  publisher={SIAM}
}
@article{huang2006covariance,
  title={Covariance matrix selection and estimation via penalised normal likelihood},
  author={Huang, Jianhua Z and Liu, Naiping and Pourahmadi, Mohsen and Liu, Linxu},
  journal={Biometrika},
  pages={85--98},
  year={2006},
  publisher={JSTOR}
}
@article{pourahmadi2000maximum,
  title={Maximum likelihood estimation of generalised linear models for multivariate normal covariance matrix},
  author={Pourahmadi, Mohsen},
  journal={Biometrika},
  pages={425--435},
  year={2000},
  publisher={JSTOR}
}
@article{pourahmadi1999joint,
  title={Joint mean-covariance models with applications to longitudinal data: Unconstrained parameterisation},
  author={Pourahmadi, Mohsen},
  journal={Biometrika},
  pages={677--690},
  year={1999},
  publisher={JSTOR}
}
@article{hoff2009hierarchical,
  title={A hierarchical eigenmodel for pooled covariance estimation},
  author={Hoff, Peter D},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={71},
  number={5},
  pages={971--992},
  year={2009},
  publisher={Wiley Online Library}
}
@article{wu2009banding,
  title={Banding sample autocovariance matrices of stationary processes},
  author={Wu, Wei Biao and Pourahmadi, Mohsen},
  journal={Statistica Sinica},
  pages={1755--1768},
  year={2009},
  publisher={JSTOR}
}
@article{karoui2008spectrum,
  title={Spectrum estimation for large dimensional covariance matrices using random matrix theory},
  author={Karoui, Noureddine El},
  journal={The Annals of Statistics},
  pages={2757--2790},
  year={2008},
  publisher={JSTOR}
}
@article{karoui2008operator,
  title={Operator norm consistent estimation of large-dimensional sparse covariance matrices},
  author={Karoui, Noureddine El},
  journal={The Annals of Statistics},
  pages={2717--2756},
  year={2008},
  publisher={JSTOR}
}
@article{bickel2008regularized,
  title={Regularized estimation of large covariance matrices},
  author={Bickel, Peter J and Levina, Elizaveta},
  journal={The Annals of Statistics},
  pages={199--227},
  year={2008},
  publisher={JSTOR}
}
@article{yuan2007model,
  title={Model selection and estimation in the Gaussian graphical model},
  author={Yuan, Ming and Lin, Yi},
  journal={Biometrika},
  pages={19--35},
  year={2007},
  publisher={JSTOR}
}
@article{meinshausen2006high,
  title={High-dimensional graphs and variable selection with the lasso},
  author={Meinshausen, Nicolai and B{\"u}hlmann, Peter},
  journal={The annals of statistics},
  pages={1436--1462},
  year={2006},
  publisher={JSTOR}
}
@article{ledoit2003flexible,
  title={Flexible multivariate GARCH modeling with an application to international stock markets},
  author={Ledoit, Olivier and Santa-Clara, Pedro and Wolf, Michael},
  journal={Review of Economics and Statistics},
  volume={85},
  number={3},
  pages={735--747},
  year={2003},
  publisher={MIT Press}
}
@book{diggle2002analysis,
  title={Analysis of longitudinal data},
  author={Diggle, Peter},
  year={2002},
  publisher={Oxford University Press}
}
@book{cressie2015statistics,
  title={Statistics for spatial data},
  author={Cressie, Noel},
  year={2015},
  publisher={John Wiley \& Sons}
}
@article{ledoit2004well,
  title={A well-conditioned estimator for large-dimensional covariance matrices},
  author={Ledoit, Olivier and Wolf, Michael},
  journal={Journal of multivariate analysis},
  volume={88},
  number={2},
  pages={365--411},
  year={2004},
  publisher={Elsevier}
}
@article{schafer2005shrinkage,
  title={A shrinkage approach to large-scale covariance matrix estimation and implications for functional genomics},
  author={Sch{\"a}fer, Juliane and Strimmer, Korbinian and others},
  journal={Statistical applications in genetics and molecular biology},
  volume={4},
  number={1},
  pages={32},
  year={2005}
}
@article{butte2000discovering,
  title={Discovering functional relationships between RNA expression and chemotherapeutic susceptibility using relevance networks},
  author={Butte, Atul J and Tamayo, Pablo and Slonim, Donna and Golub, Todd R and Kohane, Isaac S},
  journal={Proceedings of the National Academy of Sciences},
  volume={97},
  number={22},
  pages={12182--12186},
  year={2000},
  publisher={National Acad Sciences}
}
@article{fan2008high,
  title={High dimensional covariance matrix estimation using a factor model},
  author={Fan, Jianqing and Fan, Yingying and Lv, Jinchi},
  journal={Journal of Econometrics},
  volume={147},
  number={1},
  pages={186--197},
  year={2008},
  publisher={Elsevier}
}
@article{markowitz1952portfolio,
  title={Portfolio selection},
  author={Markowitz, Harry},
  journal={The journal of finance},
  volume={7},
  number={1},
  pages={77--91},
  year={1952},
  publisher={Wiley Online Library}
}
@article{zou2006sparse,
  title={Sparse principal component analysis},
  author={Zou, Hui and Hastie, Trevor and Tibshirani, Robert},
  journal={Journal of computational and graphical statistics},
  volume={15},
  number={2},
  pages={265--286},
  year={2006},
  publisher={Taylor \& Francis}
}
@book{friedman2001elements,
  title={The elements of statistical learning},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  year={2001},
  publisher={Springer series in statistics Springer, Berlin}
}
@article{friedman1989regularized,
  title={Regularized discriminant analysis},
  author={Friedman, Jerome H},
  journal={Journal of the American statistical association},
  volume={84},
  number={405},
  pages={165--175},
  year={1989},
  publisher={Taylor \& Francis}
}
@article{ideker2008protein,
  title={Protein networks in disease},
  author={Ideker, Trey and Sharan, Roded},
  journal={Genome research},
  volume={18},
  number={4},
  pages={644--652},
  year={2008},
  publisher={Cold Spring Harbor Lab}
}
@article{jimenez2001human,
  title={Human disease genes},
  author={Jimenez-Sanchez, Gerardo and Childs, Barton and Valle, David},
  journal={Nature},
  volume={409},
  number={6822},
  pages={853--855},
  year={2001},
  publisher={Nature Publishing Group}
}
@article{dasarathy2015sketching,
  title={Sketching sparse matrices, covariances, and graphs via tensor products},
  author={Dasarathy, Gautam and Shah, Parikshit and Bhaskar, Badri Narayan and Nowak, Robert D},
  journal={IEEE Transactions on Information Theory},
  volume={61},
  number={3},
  pages={1373--1388},
  year={2015},
  publisher={IEEE}
}
@article{chen2015exact,
  title={Exact and stable covariance estimation from quadratic sampling via convex programming},
  author={Chen, Yuxin and Chi, Yuejie and Goldsmith, Andrea J},
  journal={IEEE Transactions on Information Theory},
  volume={61},
  number={7},
  pages={4034--4059},
  year={2015},
  publisher={IEEE}
}
@article{cai2015rop,
  title={ROP: Matrix recovery via rank-one projections},
  author={Cai, T Tony and Zhang, Anru and others},
  journal={The Annals of Statistics},
  volume={43},
  number={1},
  pages={102--138},
  year={2015},
  publisher={Institute of Mathematical Statistics}
}
@article{fan2016overview,
  title={An overview of the estimation of large covariance and precision matrices},
  author={Fan, Jianqing and Liao, Yuan and Liu, Han},
  journal={The Econometrics Journal},
  volume={19},
  number={1},
  pages={C1--C32},
  year={2016},
  publisher={Wiley Online Library}
}
@article{cai2016estimating,
  title={Estimating structured high-dimensional covariance and precision matrices: Optimal rates and adaptive estimation},
  author={Cai, T Tony and Ren, Zhao and Zhou, Harrison H and others},
  journal={Electronic Journal of Statistics},
  volume={10},
  number={1},
  pages={1--59},
  year={2016},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{lam2009sparsistency,
  title={Sparsistency and rates of convergence in large covariance matrix estimation},
  author={Lam, Clifford and Fan, Jianqing},
  journal={Annals of statistics},
  volume={37},
  number={6B},
  pages={4254},
  year={2009},
  publisher={NIH Public Access}
}
@article{fan2016overview,
  title={An overview of the estimation of large covariance and precision matrices},
  author={Fan, Jianqing and Liao, Yuan and Liu, Han},
  journal={The Econometrics Journal},
  volume={19},
  number={1},
  pages={C1--C32},
  year={2016},
  publisher={Wiley Online Library}
}
@article{li2016sure,
  title={SURE Information Criteria for Large Covariance Matrix Estimation and Their Asymptotic Properties},
  author={Li, Danning and Zou, Hui},
  journal={IEEE Transactions on Information Theory},
  volume={62},
  number={4},
  pages={2153--2169},
  year={2016},
  publisher={IEEE}
}
@article{cai2015optimal,
  title={Optimal estimation and rank detection for sparse spiked covariance matrices},
  author={Cai, Tony and Ma, Zongming and Wu, Yihong},
  journal={Probability theory and related fields},
  volume={161},
  number={3-4},
  pages={781--815},
  year={2015},
  publisher={Springer}
}
@article{ma2013sparse,
  title={Sparse principal component analysis and iterative thresholding},
  author={Ma, Zongming and others},
  journal={The Annals of Statistics},
  volume={41},
  number={2},
  pages={772--801},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@article{paul2007asymptotics,
  title={Asymptotics of sample eigenstructure for a large dimensional spiked covariance model},
  author={Paul, Debashis},
  journal={Statistica Sinica},
  pages={1617--1642},
  year={2007},
  publisher={JSTOR}
}
@article{berthet2013optimal,
  title={Optimal detection of sparse principal components in high dimension},
  author={Berthet, Quentin and Rigollet, Philippe and others},
  journal={The Annals of Statistics},
  volume={41},
  number={4},
  pages={1780--1815},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}@article{ravikumar2011high,
  title={High-dimensional covariance estimation by minimizing $\ell$1-penalized log-determinant divergence},
  author={Ravikumar, Pradeep and Wainwright, Martin J and Raskutti, Garvesh and Yu, Bin and others},
  journal={Electronic Journal of Statistics},
  volume={5},
  pages={935--980},
  year={2011},
  publisher={The Institute of Mathematical Statistics and the Bernoulli Society}
}
@article{cai2013sparse,
  title={Sparse PCA: Optimal rates and adaptive estimation},
  author={Cai, T Tony and Ma, Zongming and Wu, Yihong and others},
  journal={The Annals of Statistics},
  volume={41},
  number={6},
  pages={3074--3110},
  year={2013},
  publisher={Institute of Mathematical Statistics}
}
@inproceedings{chandrasekaran2010latent,
  title={Latent variable graphical model selection via convex optimization},
  author={Chandrasekaran, Venkat and Parrilo, Pablo A and Willsky, Alan S},
  booktitle={Communication, Control, and Computing (Allerton), 2010 48th Annual Allerton Conference on},
  pages={1610--1613},
  year={2010},
  organization={IEEE}
}
@article{cai2011adaptive,
  title={Adaptive thresholding for sparse covariance matrix estimation},
  author={Cai, Tony and Liu, Weidong},
  journal={Journal of the American Statistical Association},
  volume={106},
  number={494},
  pages={672--684},
  year={2011},
  publisher={Taylor \& Francis}
}
@article{johnstone2012consistency,
  title={On consistency and sparsity for principal components analysis in high dimensions},
  author={Johnstone, Iain M and Lu, Arthur Yu},
  journal={Journal of the American Statistical Association},
  year={2012},
  publisher={Taylor \& Francis}
}
@article{paul2007asymptotics,
  title={Asymptotics of sample eigenstructure for a large dimensional spiked covariance model},
  author={Paul, Debashis},
  journal={Statistica Sinica},
  pages={1617--1642},
  year={2007},
  publisher={JSTOR}
}
@article{fan2014challenges,
  title={Challenges of big data analysis},
  author={Fan, Jianqing and Han, Fang and Liu, Han},
  journal={National science review},
  volume={1},
  number={2},
  pages={293--314},
  year={2014},
  publisher={Oxford University Press}
}
@article{ledoit2004well,
  title={A well-conditioned estimator for large-dimensional covariance matrices},
  author={Ledoit, Olivier and Wolf, Michael},
  journal={Journal of multivariate analysis},
  volume={88},
  number={2},
  pages={365--411},
  year={2004},
  publisher={Elsevier}
}
@article{ledoit2003improved,
  title={Improved estimation of the covariance matrix of stock returns with an application to portfolio selection},
  author={Ledoit, Olivier and Wolf, Michael},
  journal={Journal of empirical finance},
  volume={10},
  number={5},
  pages={603--621},
  year={2003},
  publisher={Elsevier}
}
@INPROCEEDINGS{West03bayesianfactor,
    author = {Mike West},
    title = {Bayesian Factor Regression Models in the "Large p, Small n" Paradigm},
    booktitle = {Bayesian Statistics},
    year = {2003},
    pages = {723--732},
    publisher = {Oxford University Press}
}
@article{lucas2006sparse,
  title={Sparse statistical modelling in gene expression genomics},
  author={Lucas, Joe and Carvalho, Carlos and Wang, Quanli and Bild, Andrea and Nevins, JR and West, Mike},
  journal={Bayesian Inference for Gene Expression and Proteomics},
  volume={1},
  pages={0--1},
  year={2006},
  publisher={Cambridge University Press, Cambridge}
}
@article{carvalho2012high,
  title={High-dimensional sparse factor modeling: applications in gene expression genomics},
  author={Carvalho, Carlos M and Chang, Jeffrey and Lucas, Joseph E and Nevins, Joseph R and Wang, Quanli and West, Mike},
  journal={Journal of the American Statistical Association},
  year={2012},
  publisher={Taylor \& Francis}
}
@book{friedman2001elements,
  title={The elements of statistical learning},
  author={Friedman, Jerome and Hastie, Trevor and Tibshirani, Robert},
  volume={1},
  year={2001},
  publisher={Springer series in statistics Springer, Berlin}
}
@article{efron1986biased,
  title={How biased is the apparent error rate of a prediction rule?},
  author={Efron, Bradley},
  journal={Journal of the American Statistical Association},
  volume={81},
  number={394},
  pages={461--470},
  year={1986},
  publisher={Taylor \& Francis}
}
@article{efron2004estimation,
  title={The estimation of prediction error},
  author={Efron, Bradley},
  journal={Journal of the American Statistical Association},
  volume={99},
  number={467},
  year={2004}
}
@article{stein1981estimation,
  title={Estimation of the mean of a multivariate normal distribution},
  author={Stein, Charles M},
  journal={The annals of Statistics},
  pages={1135--1151},
  year={1981},
  publisher={JSTOR}
}
@article{li2014asymptotic,
  title={Asymptotic Properties of SURE Information Criteria for Large Covariance Matrices},
  author={Li, Danning and Zou, Hui},
  journal={arXiv preprint arXiv:1406.6514},
  year={2014}
}
@article{xiao2014theoretic,
  title={On the theoretic and practical merits of the banding estimator for large covariance matrices},
  author={Xiao, Luo and Bunea, Florentina},
  journal={arXiv preprint arXiv:1402.0844},
  year={2014}
}
@article{bickel2008regularized,
  title={Regularized estimation of large covariance matrices},
  author={Bickel, Peter J and Levina, Elizaveta},
  journal={The Annals of Statistics},
  pages={199--227},
  year={2008},
  publisher={JSTOR}
}
@article{yi2013sure,
  title={SURE-tuned tapering estimation of large covariance matrices},
  author={Yi, Feng and Zou, Hui},
  journal={Computational Statistics \& Data Analysis},
  volume={58},
  pages={339--351},
  year={2013},
  publisher={Elsevier}
}
@article{donoho1995adapting,
  title={Adapting to unknown smoothness via wavelet shrinkage},
  author={Donoho, David L and Johnstone, Iain M},
  journal={Journal of the american statistical association},
  volume={90},
  number={432},
  pages={1200--1224},
  year={1995},
  publisher={Taylor \& Francis Group}
}
@article{zou2007degrees,
  title={On the “degrees of freedom” of the lasso},
  author={Zou, Hui and Hastie, Trevor and Tibshirani, Robert and others},
  journal={The Annals of Statistics},
  volume={35},
  number={5},
  pages={2173--2192},
  year={2007},
  publisher={Institute of Mathematical Statistics}
}
@article{johnstone2001distribution,
  title={On the distribution of the largest eigenvalue in principal components analysis},
  author={Johnstone, Iain M},
  journal={Annals of statistics},
  pages={295--327},
  year={2001},
  publisher={JSTOR}
}
@article{wu2003nonparametric,
  title={Nonparametric estimation of large covariance matrices of longitudinal data},
  author={Wu, Wei Biao and Pourahmadi, Mohsen},
  journal={Biometrika},
  volume={90},
  number={4},
  pages={831--844},
  year={2003},
  publisher={Biometrika Trust}
}
@article{furrer2007estimation,
  title={Estimation of high-dimensional prior and posterior covariance matrices in Kalman filter variants},
  author={Furrer, Reinhard and Bengtsson, Thomas},
  journal={Journal of Multivariate Analysis},
  volume={98},
  number={2},
  pages={227--255},
  year={2007},
  publisher={Elsevier}
}
@article{cai2012optimal,
  title={Optimal rates of convergence for sparse covariance matrix estimation},
  author={Cai, T Tony and Zhou, Harrison H and others},
  journal={The Annals of Statistics},
  volume={40},
  number={5},
  pages={2389--2420},
  year={2012},
  publisher={Institute of Mathematical Statistics}
}
@article{cai2010optimal,
  title={Optimal rates of convergence for covariance matrix estimation},
  author={Cai, T Tony and Zhang, Cun-Hui and Zhou, Harrison H and others},
  journal={The Annals of Statistics},
  volume={38},
  number={4},
  pages={2118--2144},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}
@article{bickel2008covariance,
  title={Covariance regularization by thresholding},
  author={Bickel, Peter J and Levina, Elizaveta},
  journal={The Annals of Statistics},
  pages={2577--2604},
  year={2008},
  publisher={JSTOR}
}
@article{cai2011adaptive,
  title={Adaptive thresholding for sparse covariance matrix estimation},
  author={Cai, Tony and Liu, Weidong},
  journal={Journal of the American Statistical Association},
  volume={106},
  number={494},
  pages={672--684},
  year={2011},
  publisher={Taylor \& Francis}
}
@article{karoui2008operator,
  title={Operator norm consistent estimation of large-dimensional sparse covariance matrices},
  author={Karoui, Noureddine El},
  journal={The Annals of Statistics},
  pages={2717--2756},
  year={2008},
  publisher={JSTOR}
}
@article{rothman2009generalized,
  title={Generalized thresholding of large covariance matrices},
  author={Rothman, Adam J and Levina, Elizaveta and Zhu, Ji},
  journal={Journal of the American Statistical Association},
  volume={104},
  number={485},
  pages={177--186},
  year={2009},
  publisher={Taylor \& Francis}
}
@article{bai2011estimating,
  title={Estimating high dimensional covariance matrices and its applications},
  author={Bai, Jushan and Shi, Shuzhong},
  year={2011}
}

@article{bai2002determining,
  title={Determining the number of factors in approximate factor models},
  author={Bai, Jushan and Ng, Serena},
  journal={Econometrica},
  volume={70},
  number={1},
  pages={191--221},
  year={2002},
  publisher={Wiley Online Library}
}

@article{amengual2007consistent,
  title={Consistent estimation of the number of dynamic factors in a large N and T panel},
  author={Amengual, Dante and Watson, Mark W},
  journal={Journal of Business \& Economic Statistics},
  volume={25},
  number={1},
  pages={91--96},
  year={2007},
  publisher={Taylor \& Francis}
}


@article{shao2011sparse,
  title={Sparse linear discriminant analysis by thresholding for high dimensional data},
  author={Shao, Jun and Wang, Yazhen and Deng, Xinwei and Wang, Sijian and others},
  journal={The Annals of statistics},
  volume={39},
  number={2},
  pages={1241--1265},
  year={2011},
  publisher={Institute of Mathematical Statistics}
}
@article{bhattacharya2011sparse,
  title={Sparse Bayesian infinite factor models},
  author={Bhattacharya, Anirban and Dunson, David B},
  journal={Biometrika},
  volume={98},
  number={2},
  pages={291},
  year={2011}
}
@article{marvcenko1967distribution,
  title={Distribution of eigenvalues for some sets of random matrices},
  author={Mar{\v{c}}enko, Vladimir A and Pastur, Leonid Andreevich},
  journal={Sbornik: Mathematics},
  volume={1},
  number={4},
  pages={457--483},
  year={1967},
  publisher={Turpion Ltd}
}
@article{pati2014posterior,
  title={Posterior contraction in sparse Bayesian factor models for massive covariance matrices},
  author={Pati, Debdeep and Bhattacharya, Anirban and Pillai, Natesh S and Dunson, David B},
  journal={The Annals of Statistics},
  volume={42},
  number={3},
  pages={1102--1130},
  year={2014},
  publisher={Institute of Mathematical Statistics}
}
@article{bunea2015sample,
  title={On the sample covariance matrix estimator of reduced effective rank population matrices, with applications to fPCA},
  author={Bunea, Florentina and Xiao, Luo},
  journal={Bernoulli},
  volume={21},
  number={2},
  pages={1200--1230},
  year={2015},
  publisher={Bernoulli Society for Mathematical Statistics and Probability}
}
@article{pourahmadi2011covariance,
  title={Covariance estimation: The GLM and regularization perspectives},
  author={Pourahmadi, Mohsen},
  journal={Statistical Science},
  pages={369--387},
  year={2011},
  publisher={JSTOR}
}
@article{cai2010optimal,
  title={Optimal rates of convergence for covariance matrix estimation},
  author={Cai, T Tony and Zhang, Cun-Hui and Zhou, Harrison H},
  journal={The Annals of Statistics},
  volume={38},
  number={4},
  pages={2118--2144},
  year={2010},
  publisher={Institute of Mathematical Statistics}
}
@article{wu2003nonparametric,
  title={Nonparametric estimation of large covariance matrices of longitudinal data},
  author={Wu, Wei Biao and Pourahmadi, Mohsen},
  journal={Biometrika},
  volume={90},
  number={4},
  pages={831--844},
  year={2003},
  publisher={Biometrika Trust}
}
@article{rothman2009generalized,
  title={Generalized thresholding of large covariance matrices},
  author={Rothman, Adam J and Levina, Elizaveta and Zhu, Ji},
  journal={Journal of the American Statistical Association},
  volume={104},
  number={485},
  pages={177--186},
  year={2009},
  publisher={Taylor \& Francis}
}
@article{johnstone2004sparse,
  title={Sparse principal components analysis},
  author={Johnstone, Iain M and Lu, Arthur Yu},
  journal={Unpublished manuscript},
  volume={7},
  year={2004}
}
@article{fan2013large,
  title={Large covariance estimation by thresholding principal orthogonal complements},
  author={Fan, Jianqing and Liao, Yuan and Mincheva, Martina},
  journal={Journal of the Royal Statistical Society: Series B (Statistical Methodology)},
  volume={75},
  number={4},
  pages={603--680},
  year={2013},
  publisher={Wiley Online Library}
}
@article{guhaniyogi2013bayesian,
  title={Bayesian Compressed Regression},
  author={Guhaniyogi, Rajarshi and Dunson, David B},
  journal={arXiv preprint arXiv:1303.0642},
  year={2013}
}
@article{banerjee2012efficient,
  title={Efficient Gaussian process regression for large datasets},
  author={Banerjee, Anjishnu and Dunson, David B and Tokdar, Surya T},
  journal={Biometrika},
  pages={ass068},
  year={2012},
  publisher={Biometrika Trust}
}
@article{azizyan2015extreme,
  title={Extreme compressive sampling for covariance estimation},
  author={Azizyan, Martin and Krishnamurthy, Akshay and Singh, Aarti},
  journal={arXiv preprint arXiv:1506.00898},
  year={2015}
}
@article{marzetta2011random,
  title={A random matrix-theoretic approach to handling singular covariance estimates},
  author={Marzetta, Thomas L and Tucci, Gabriel H and Simon, Steven H},
  journal={Information Theory, IEEE Transactions on},
  volume={57},
  number={9},
  pages={6256--6271},
  year={2011},
  publisher={IEEE}
}
@book{saulis2012limit,
  title={Limit theorems for large deviations},
  author={Saulis, Leonas and Statulevicius, VA},
  volume={73},
  year={2012},
  publisher={Springer Science \& Business Media}
}
@article{ledoit2004well,
  title={A well-conditioned estimator for large-dimensional covariance matrices},
  author={Ledoit, Olivier and Wolf, Michael},
  journal={Journal of multivariate analysis},
  volume={88},
  number={2},
  pages={365--411},
  year={2004},
  publisher={Elsevier}
}
@article{haff1980empirical,
  title={Empirical Bayes estimation of the multivariate normal covariance matrix},
  author={Haff, LR},
  journal={The Annals of Statistics},
  pages={586--597},
  year={1980},
  publisher={JSTOR}
}
@book{efron2012large,
  title={Large-scale inference: empirical Bayes methods for estimation, testing, and prediction},
  author={Efron, Bradley},
  volume={1},
  year={2012},
  publisher={Cambridge University Press}
}
@article{xue2012positive,
  title={Positive-definite ℓ1-penalized estimation of large covariance matrices},
  author={Xue, Lingzhou and Ma, Shiqian and Zou, Hui},
  journal={Journal of the American Statistical Association},
  volume={107},
  number={500},
  pages={1480--1491},
  year={2012},
  publisher={Taylor \& Francis Group}
}
 @inproceedings{stein1956inadmissibility,
  title={Inadmissibility of the usual estimator for the mean of a multivariate normal distribution},
  author={Stein, Charles and others},
  booktitle={Proceedings of the Third Berkeley symposium on mathematical statistics and probability},
  volume={1},
  number={399},
  pages={197--206},
  year={1956}
}
